Taming Generative Diffusion Prior for Universal Blind Image Restoration

Diffusion models have been widely utilized for image restoration. However, previous blind image restoration methods still need to assume the type of degradation model while leaving the parameters to be optimized, limiting their real-world applications. Therefore, we aim to tame generative diffusion prior for universal blind image restoration dubbed BIR-D, which utilizes an optimizable convolutional kernel to simulate the degradation model and dynamically update the parameters of the kernel in the diffusion steps, enabling it to achieve blind image restoration results even in various complex situations. Besides, based on mathematical reasoning, we have provided an empirical formula for the chosen of adaptive guidance scale, eliminating the need for a grid search for the optimal parameter. Experimentally, Our BIR-D has demonstrated superior practicality and versatility than off-the-shelf unsupervised methods across various tasks both on real-world and synthetic datasets, qualitatively and quantitatively. BIR-D is able to fulfill multi-guidance blind image restoration. Moreover, BIR-D can also restore images that undergo multiple and complicated degradations, demonstrating the practical applications.

==> Sections/Limitation_and_Future_Works.tex <==
\section{Limitation and Future Works}
\label{limitation}
Since we utilize a single pre-trained unconditional diffusion model provided by~\cite{dhariwal2021diffusion}, the generation speed will increase when dealing with image size increasing due to the patch-based solution.
In the future, it is a very promising direction to use stable diffusion to achieve faster speed in large-size image restoration.
\clearpage
